HealthGuard: A Machine Learning-Based Security Framework for Smart Healthcare Systems

The integration of Internet-of-Things and pervasive computing in medical devices have made the modern healthcare system "smart". Today, the function of the healthcare system is not limited to treat the patients only. With the help of implantable medical devices and wearables, Smart Healthcare System (SHS) can continuously monitor different vital signs of a patient and automatically detect and prevent critical medical conditions. However, these increasing functionalities of SHS raise several security concerns and attackers can exploit the SHS in numerous ways: they can impede normal function of the SHS, inject false data to change vital signs, and tamper a medical device to change the outcome of a medical emergency. In this paper, we propose HealthGuard, a novel machine learning-based security framework to detect malicious activities in a SHS. HealthGuard observes the vital signs of different connected devices of a SHS and correlates the vitals to understand the changes in body functions of the patient to distinguish benign and malicious activities. HealthGuard utilizes four different machine learning-based detection techniques (Artificial Neural Network, Decision Tree, Random Forest, k-Nearest Neighbor) to detect malicious activities in a SHS. We trained HealthGuard with data collected for eight different smart medical devices for twelve benign events including seven normal user activities and five disease-affected events. Furthermore, we evaluated the performance of HealthGuard against three different malicious threats. Our extensive evaluation shows that HealthGuard is an effective security framework for SHS with an accuracy of 91% and an F-1 score of 90%.

==> Discussion.tex <==
\section{Discussion and Limitations} \label{sec:discussion}
In this section, we discuss the benefits and the limitations of HealthGuard in detecting malicious activities in SHSs. We also highlight some future research directions that can help to understand the threats and build secure SHSs.

\begin{itemize}
    
\item Real-life patient monitoring data: We have collected our dataset for different healthcare devices considering all the devices are connected to a patient for health monitoring. However, the collected data are not from the same patient which may introduce some false positive and false negative cases in the framework. It is also very challenging and expensive to create a real-life testbed to collect data and train HealthGuard. In the future, we would like to implement HealthGuard in a real-life smart healthcare system and test with real devices.
    %it's not real user data that means not from the same patient we are getting all the devices output. In a SHS, it's challenging and expensive to connect all the devices into a human body and to get real user data for our solution.
    
    
\item Continuous healthcare monitoring: In a SHS, a patient is monitored 24/7. In healthcare, some of the devices are used for continuous monitoring and give continuous data for the patient where some of the devices are used in a certain time interval to check the health status. So, it's a 24/7 health monitoring system and in our framework timestamp is a big challenge to implement our solution. We did consider our data is coming at different time frame and it's a continuous monitoring process.
    
\item Diverse configuration: In a SHS, number of connected devices may vary with the need of the patient/user. To evaluate HealthGuard, we consider a set of eight smart medical devices in the SHS. In reality, the number and the combination of the devices may vary which can affect the performance of HealthGuard. In addition, new smart medical devices can measure more than one vital signs at once~\cite{fit}. In future, we wi
l implement and test HealthGuard in real-life SHS with different configuration to understand the effectiveness thoroughly. l
%We have considered that for every body part there is an individual monitoring device. For example, for heart-rate monitor, there is an ECG device. Similarly, for blood pressure and respiratory monitoring, there are two different devices. But it's not right all the time as for smart medical devices one device can do more than one monitoring at the same time. For instance, there are so many devices which can track heart-rate, sleep monitoring at the same time \cite{fit}.
    
\item Performance Overhead: As we used MATLAB and Scikit-Learn toolbox for Python to build our framework, HealthGuard runs in the local machine which does not demonstrate any overhead. Moreover, we collected real-life data for eight different devices from publicly available dataset which does not illustrate any overhead of collecting data. In future, we would like to evaluate HealthGuard in a real-life settings to calculate the overhead and perform a detailed evaluation.
\end{itemize}

 Although our proposed security framework (HealthGuard) can detect threats in a smart healthcare system, we will expand this solution in a real-life environment with a real-life health monitoring system.


